Refinement Types for TypeScript

We present Refined TypeScript (RSC), a lightweight refinement type system for TypeScript, that enables static verification of higher-order, imperative programs. We develop a formal core of RSC that delineates the interaction between refinement types and mutability. Next, we extend the core to account for the imperative and dynamic features of TypeScript. Finally, we evaluate RSC on a set of real world benchmarks, including parts of the Octane benchmarks, D3, Transducers, and the TypeScript compiler.

==> 0X-transducers.tex <==
\section{Transducers (A Case Study)}\label{sec:transducers}

We now delve deeper into one of our benchmarks: the Transducers
library. At its heart this library is about reducing collections, aka
performing folds. A Transformer is anything that implements three
functions: @init@ to begin computation, @step@ to consume one element
from an input collection, and @result@ to perform any post-processing.
One could imagine rewriting @reduce@ from Figure 1 by building a
Transformer where @init@ returns @x@, @step@ invokes @f@, and @result@
is the identity.  \footnote{For simplicity of discussion we will
henceforth ignore init and initialization in general, as well as some
other details.} The Transformers provided by the library are
composable - their constructors take, as a final argument, another
Transformer, and then all calls to the outer Transformer's functions
invoke the corresponding one of the inner Transformer. This gives rise
to the concept of a Transducer, a function of type @Transformer ->
Transformer@ and this library's namesake.

The main reason this library interests us is because some of its
functions are massively overloaded. Consider, for example, the
@reduce@ function it defines. As  discussed above, @reduce@ needs a
Transformer and a collection. There are two opportunities for
overloading here. First of all, the main ways that a Transformer is
more general than a simple step function is that it can be stateful
and that it defines the @result@ post-processing step. Most of the
time the user does not need these features, in which case their
Transformer is just a wrapper around a step function. Thus for
convenience, the user is allowed to pass in either a full-fledged
Transformer or a step function which will automatically get wrapped
into one. Secondly, the collection being reduced can be a stunning
array of options: an Array, a string (\ie a collection of characters,
which are themselves just strings), an arbitrary object (\ie, in
Javascript, a collection of key-value pairs), an iterator (an object
that defines a @next@ function that iterates through the collection),
or an iterable (an object that defines an @iterator@ function that
returns an iterator). Each of these collections needs to be dispatched
to a type-specific reduce function that knows how to iterate over that
kind of collection. In each overload, the type of the collection must
match the type of the Transformer or step function. Thus our @reduce@
begins as follows:

\begin{code}
/*@ /\ (B -> A -> B)          -> A[]    -> B 
    /\ Transformer<A,B>       -> A[]    -> B 
    /\ (B -> string -> B)     -> string -> B
    /\ Transformer<string, B> -> string -> B 
    ... */
function reduce(xf, coll) {
  xf = typeof xf == "function" ? wrap(xf) : xf;
  if(isString(coll)) {
      return stringReduce(xf, coll);
  } else if(isArray(coll)) {
      return arrayReduce(xf, coll);
  } else...
\end{code}

If you count all 5 types of collection and the 2 options for step
function vs Transformer, this function has 10 distinct overloads!
Another similar function offers 5 choices of input collection and 3
choices of output collection for a total of 15 distinct overloads.

